Search-Based Task and Motion Planning for Hybrid Systems: Agile Autonomous Vehicles

To achieve optimal robot behavior in dynamic scenarios we need to consider complex dynamics in a predictive manner. In the vehicle dynamics community, it is well know that to achieve time-optimal driving on low surface, the vehicle should utilize drifting. Hence many authors have devised rules to split circuits and employ drifting on some segments. These rules are suboptimal and do not generalize to arbitrary circuit shapes (e.g., S-like curves). So, the question "When to go into which mode and how to drive in it?" remains unanswered. To choose the suitable mode (discrete decision), the algorithm needs information about the feasibility of the continuous motion in that mode. This makes it a class of Task and Motion Planning (TAMP) problems, which are known to be hard to solve optimally in real-time. In the AI planning community, search methods are commonly used. However, they cannot be directly applied to TAMP problems due to the continuous component. Here, we present a search-based method that effectively solves this problem and efficiently searches in a highly dimensional state space with nonlinear and unstable dynamics. The space of the possible trajectories is explored by sampling different combinations of motion primitives guided by the search. Our approach allows to use multiple locally approximated models to generate motion primitives (e.g., learned models of drifting) and effectively simplify the problem without losing accuracy. The algorithm performance is evaluated in simulated driving on a mixed-track with segments of different curvatures (right and left). Our code is available at https://git.io/JenvB

==> figures/3_perfdrive_prob2.tex <==
\usetikzlibrary{decorations,decorations.markings} 
\pgfkeys{/tikz/.cd,
    street mark distance/.store in=\StreetMarkDistance,
    street mark distance=10pt,
    street mark step/.store in=\StreetMarkStep,
    street mark step=1pt,
}

\pgfdeclaredecoration{street mark}{initial}
{% 
\state{initial}[width=\StreetMarkStep,next state=cont] {
    \pgfmoveto{\pgfpoint{\StreetMarkStep}{\StreetMarkDistance}}
    \pgfpathlineto{\pgfpoint{0.3\pgflinewidth}{\StreetMarkDistance}}
    \pgfcoordinate{lastup}{\pgfpoint{1pt}{\StreetMarkDistance}}
    \xdef\marmotarrowstart{0}
  }
  \state{cont}[width=\StreetMarkStep]{
     \pgfmoveto{\pgfpointanchor{lastup}{center}}
     \pgfpathlineto{\pgfpoint{\StreetMarkStep}{\StreetMarkDistance}}
     \pgfcoordinate{lastup}{\pgfpoint{\StreetMarkStep}{\StreetMarkDistance}}
  }
  \state{final}[width=\StreetMarkStep]
  { % perhaps unnecessary but doesn't hurt either
    \pgfmoveto{\pgfpointdecoratedpathlast}
  }
}


\tikzset{
    car_top/.pic={
    
    %Car body
\filldraw [black, fill=#1, very thin] plot[smooth, black, tension=.7, very thin] 
	coordinates {(2.3248,0) (2.2967,0.4058) (2.0941,0.7925)(1.7847,0.9958) (1.1874,1.0261) (0.9497,1.0108)}
	.. controls (0.9124,1.143) and (0.8648,1.2352) .. (0.7463,1.1888) .. controls (0.7628,1.0703) and (0.7832,1.0089) .. (0.8202,0.952) .. controls (0.6029,0.9902) and (0.1582,1.0079) .. (-0.2536,0.9816) .. controls (-0.3325,1.0605) and (-0.4289,1.0459) .. (-0.5136,0.9787) .. controls (-0.6947,0.9904) and (-0.8232,0.9758) .. (-0.94,0.9524)
	plot[smooth, tension=.7,very thin] coordinates {(-0.94,0.9524)(-1.1951,1.0129) (-1.8081,0.9951) (-2.1686,0.8328) (-2.3894,0.4889) (-2.4286,0) };

\fill [fill=#1,very thin](-2.4286,0)--(-0.94,0.9524)--(2.3248,0)--(-0.94,-0.9524);

\filldraw  [black, fill=#1, very thin] plot[smooth, black, tension=.7,very thin] 
	coordinates {(2.3248,0) (2.2967,-0.4058) (2.0941,-0.7925)(1.7847,-0.9958) (1.1874,-1.0261) (0.9497,-1.0108)}
	.. controls (0.9124,-1.143) and (0.8648,-1.2352) .. (0.7463,-1.1888) .. controls (0.7628,-1.0703) and (0.7832,-1.0089) .. (0.8202,-0.952) .. controls (0.6029,-0.9902) and (0.1582,-1.0079) .. (-0.2536,-0.9816) .. controls (-0.3325,-1.0605) and (-0.4289,-1.0459) .. (-0.5136,-0.9787) .. controls (-0.6947,-0.9904) and (-0.8232,-0.9758) .. (-0.94,-0.9524)
	plot[smooth, tension=.7,very thin] coordinates {(-0.94,-0.9524)(-1.1951,-1.0129) (-1.8081,-0.9951) (-2.1686,-0.8328) (-2.3894,-0.4889) (-2.4286,0) };

%Front window
\draw [smooth cycle, black, fill=darkgray,very thin](0.52,0.75) .. controls (0.7,0.78) and (1,0.82) .. (1.2,0.85) .. controls (1.7,0.5) and (1.7,-0.5) .. (1.2,-0.85) .. controls (1,-0.82) and (0.7,-0.78) .. (0.52,-0.75) .. controls (0.7,-0.25) and (0.7,0.25) .. (0.52,0.75);
%Back window
\draw [smooth cycle, black, fill=darkgray,very thin](-1.06,0.67) .. controls (-1.33,0.68) and (-1.57,0.67) .. (-1.8,0.68) .. controls (-2.1,0.27) and (-2.1,-0.27) .. (-1.8,-0.68) .. controls (-1.57,-0.67) and (-1.33,-0.68) .. (-1.06,-0.67) .. controls (-1.16,-0.3) and (-1.16,0.3) .. (-1.06,0.67);
%windows
\draw [smooth cycle, black, fill=darkgray,very thin](0.97,0.87) .. controls (0.32,1) and (-0.84,0.93) .. (-1.47,0.83) .. controls (-1.23,0.8) and (-1.0974,0.7863) .. (-0.88,0.76) .. controls (-0.56,0.75) and (0.02,0.76) .. (0.4,0.78) .. controls (0.63,0.82) and (0.7,0.83) .. (0.97,0.87);
\draw [smooth cycle, black, fill=darkgray,very thin](0.97,-0.87) .. controls (0.32,-1) and (-0.84,-0.93) .. (-1.47,-0.83) .. controls (-1.23,-0.8) and (-1.0974,-0.7863) .. (-0.88,-0.76) .. controls (-0.56,-0.75) and (0.02,-0.76) .. (0.4,-0.78) .. controls (0.63,-0.82) and (0.7,-0.83) .. (0.97,-0.87);

%back lights
\draw [rotate=51, black, fill=red, very thin] (-0.75,2.07) ellipse (0.18 and 0.06);
\draw [rotate=-51, black, fill=red, very thin] (-0.75,-2.07) ellipse (0.18 and 0.06);
%front lights
\draw [rotate=-51, black, fill=white, very thin] (0.6696,2.0406) ellipse (0.19 and 0.05);
\draw [rotate=51, black, fill=white, very thin] (0.6696,-2.0406) ellipse (0.19 and 0.05);
 }}
 

%expand_bic
\tikzset{
    expand_bic/.pic={
    
    %  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0:60:1);

 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.45] {car_top={blue}} ;
      }}}]
     (0,0) arc (0:25:3) node (a){};
 \node  [valnode]  at (a) {};
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%       (0,0) arc (0:8:8) node (a){};
%  \node  [valnode]  at (a) {};
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) -- (0,1.3) node (a){};
 \node  [valnode]  at (a) {};
     
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:172:8) node (a){};
%  \node  [valnode]  at (a) {};
     
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0+180:155:3) node (a){};
 \node  [valnode]  at (a) {};

     %  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:120:1) node (a){};
%  \node  [valnode]  at (a) {};

%%
%druga velocity

 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0:30:4.5) node (a){};
 \node  [valnode]  at (a) {};

 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) -- (0,2.4) node (a){};
 \node  [valnode]  at (a) {};
    
     
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0+180:150:4.5) node (a){};
 \node  [valnode]  at (a) {};

 }}

%expand_sur
\tikzset{
    expand_sur/.pic={
    
    %  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0:60:1);

 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1+10, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0:40:1.5) node (a){};
 \node  [valnode]  at (a) {};
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1+10, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
      (0,0) arc (0:7.5:8) node (a){};
 \node  [valnode]  at (a) {};
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) -- (0,1.3) node (a){};
%  \node  [valnode]  at (a) {};
     
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:172:8) node (a){};
%  \node  [valnode]  at (a) {};
     
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:155:3) node (a){};
%  \node  [valnode]  at (a) {};

     %  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:120:1) node (a){};
%  \node  [valnode]  at (a) {};

%%
%druga velocity
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1+10, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0:55:2.2) node (a){};
 \node  [valnode]  at (a) {};
 
 \draw [red, 
  postaction={
    decorate,
    decoration={
      markings,
      mark=between positions 1 and 1 step 0.125 with
      {\pic[transform shape,rotate=#1+10, scale=0.15, opacity=0.25] {car_top={blue}} ;
      }}}]
     (0,0) arc (0:25:4.5) node (a){};
 \node  [valnode]  at (a) {};

%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) -- (0,2.4) node (a){};
%  \node  [valnode]  at (a) {};
%     
%      
%  \draw [red, 
%   postaction={
%     decorate,
%     decoration={
%       markings,
%       mark=between positions 1 and 1 step 0.125 with
%       {\pic[transform shape,rotate=#1, scale=0.15, opacity=0.25] {car_top={blue}} ;
%       }}}]
%      (0,0) arc (0+180:150:4.5) node (a){};
%  \node  [valnode]  at (a) {};

 }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\testpath}{(0,0) to[out=0,in=-90] (5,2) to[out=90,in=0] (0,4)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{tikzpicture}
  [level distance=10mm,
	 valnode/.style={color=red, fill=red, circle, draw,inner sep=1pt,outer sep=0},
	 clnode/.style={color=green, fill=green, circle, draw,inner sep=1.2pt,outer sep=0},
	 colnode/.style={color=red, fill=red, cross out, draw,inner sep=4pt,outer sep=0pt, line width =2},]
    %\path[fill=green!50!black] (0,-1.0) rectangle (7,5.0);%background
    \draw[line width=30,brown] \testpath; % asphalt
    \draw[draw=black, line width = 0.2,dashed,double distance=0] \testpath; % dashed
    \draw[yellow,decorate,decoration={street mark},street mark distance=13] \testpath; %left line
    \draw[white,decorate,decoration={street mark},street mark distance=-13] \testpath; %right line

  


%%%%%%%%%%%%%%%%%%%%%%%%

 \pic [scale=0.15, rotate=5, opacity=1] (nI) at  (1.4,0) {car_top={blue}} ;
\node []  (nI) at (1.4,0) {};
% \node [yshift =8, xshift =-4] at (nI) {$n_I$};


 
%  %
%  % expand_bic 1, rotate -90
%  \pic [scale=1, rotate=-85, opacity=1] (b) at (1.4,0) {expand_bic={0}} ;
%  
%  
%  %collision nodes
%  \node [colnode] (a) at (3.5975,0.7897) {};
%  \node [colnode] (a) at (3.7104,-0.4176) {};
% 
%  \node  [clnode]  at (nI) {};
% 
% 
%  %
%   % expand_bic 2, rotate -90
%  \pic [scale=1, rotate=-85, opacity=1]  (b) at (3.8,0.21) {expand_bic={0}} ; 
%   %collision nodes
%  \node [colnode] (a) at (5.0958,0.3347) {};
%  \node [colnode] (a) at (5.0899,0.0431) {}; %collision nodes
%  \node [colnode] (a) at (5.0276,0.5975) {};
%  \node [colnode] (a) at (6.0827,-0.2002) {}; %collision nodes
%  \node [colnode] (a) at (5.9912,0.9965) {};
%  \node [colnode] (a) at (6.1606,0.413) {};
%   %close    
%  \node  [clnode] at (3.8,0.21) {};
%   
%   % expand_bic 3, rotate -90  
%    
%  \pic [scale=1, rotate=-85, opacity=1]  (n1) at (2.7,0.1) {expand_bic={20}} ; 
%   %collision nodes
%  \node [colnode] (a) at (5.0958,0.3347) {};
%  \node [colnode] (a) at (4.9889,-0.2969) {}; %collision nodes
%  \node [colnode] (a) at (3.9849,-0.059) {};
%   %close    
%  \node  [clnode] at (2.7,0.1) {};
%  
%  %   
%   % expand_bic 4, rotate -90  
%    
%  \pic [scale=1, rotate=-55, opacity=1]  (b) at (4.9,0.9) {expand_bic={40}} ; 
%   %collision nodes
%  \node [colnode] (a) at (6.3714,2.6863) {};
%  \node [colnode] (a) at (6.0829,1.391) {}; %collision nodes
%  \node [colnode] (a) at (5.7742,1.8262) {};
%  \node [colnode] (a) at (6.8401,2.2593) {};
%  \node [colnode] (a) at (7.0673,1.6977) {}; %collision nodes
%  \node [colnode] (a) at (5.9425,1.6243) {};
%   %close    
%  \node  [clnode] at (4.9,0.9) {};
%  
%   %   
%   % expand_bic 5, rotate -90  
%    
%  \pic [scale=1, rotate=-50, opacity=1]  (n2) at (3.94,0.49) {expand_bic={40}} ; 
%   %collision nodes
%  \node [colnode] (a) at (5.7775,2.0222) {}; %collision nodes
%  \node [colnode] (a) at (6.0429,1.4669) {};
%   %close    
%  \node  [clnode] at (3.94,0.49) {};
 
 %Final
  %close    
 \node  (n3) at (4.8316,2) {};
 
  % orient 0
\draw[black, opacity=0,thin,    postaction={ decorate,  decoration={  markings,   mark=between positions 0.1245 and 0.25 step 0.1245 with   {\pic[transform shape,rotate=0, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
(nI) .. controls (1.8218,0.006) and (2.3326,0.0646) .. (2.7,0.1) .. controls (3.196,0.158) and (3.5049,0.2405) .. (3.94,0.49) .. controls (4.4275,0.7886) and (4.6994,1.03) .. (n3);
 % orient 10
\draw[black, opacity=0,thin,   postaction={ decorate,  decoration={  markings,   mark=between positions .3735 and 0.49 step 0.1245 with   {\pic[transform shape,rotate=10, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
(nI) .. controls (1.8218,0.006) and (2.3326,0.0646) .. (2.7,0.1) .. controls (3.196,0.158) and (3.5049,0.2405) .. (3.94,0.49) .. controls (4.4275,0.7886) and (4.6994,1.03) .. (n3);
 % orient 20
\draw[black, opacity=0,thin,     postaction={ decorate,  decoration={  markings,   mark=between positions .498 and .74 step 0.1245 with   {\pic[transform shape,rotate=20, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
(nI) .. controls (1.8218,0.006) and (2.3326,0.0646) .. (2.7,0.1) .. controls (3.196,0.158) and (3.5049,0.2405) .. (3.94,0.49) .. controls (4.4275,0.7886) and (4.6994,1.03) .. (n3);
 % orient 30
\draw[black, opacity=0,thin,    postaction={ decorate,  decoration={  markings,   mark=between positions .747 and .9 step 0.1245 with   {\pic[transform shape,rotate=30, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
(nI) .. controls (1.8218,0.006) and (2.3326,0.0646) .. (2.7,0.1) .. controls (3.196,0.158) and (3.5049,0.2405) .. (3.94,0.49) .. controls (4.4275,0.7886) and (4.6994,1.03) .. (n3);
 % orient 40
\draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions .9960 and 1 step 0.1245 with   {\pic[transform shape,rotate=40, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
(nI) .. controls (1.8218,0.006) and (2.3326,0.0646) .. (2.7,0.1) .. controls (3.196,0.158) and (3.5049,0.2405) .. (3.94,0.49) .. controls (4.4275,0.7886) and (4.6994,1.03) .. (n3);
 %upper half
 \draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions 0.751 and 1 step 0.1245 with   {\pic[transform shape,rotate=0, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
 (n3) .. controls (4.6148,3.0594)  and(3.9718,3.285) .. (3.6391,3.5047) .. controls (3.3496,3.6104) and (3.0856,3.7212) .. (2.6522,3.8353) .. controls (2.2454,3.8856) and (1.8886,3.8959) .. (1.4,3.9429);
 \draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions 0.6265 and .7 step 0.1245 with   {\pic[transform shape,rotate=10, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
 (n3) .. controls (4.6148,3.0594)  and(3.9718,3.285) .. (3.6391,3.5047) .. controls (3.3496,3.6104) and (3.0856,3.7212) .. (2.6522,3.8353) .. controls (2.2454,3.8856) and (1.8886,3.8959) .. (1.4,3.9429);
 \draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions .3775 and 0.6 step 0.1245 with   {\pic[transform shape,rotate=20, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
 (n3) .. controls (4.6148,3.0594)  and(3.9718,3.285) .. (3.6391,3.5047) .. controls (3.3496,3.6104) and (3.0856,3.7212) .. (2.6522,3.8353) .. controls (2.2454,3.8856) and (1.8886,3.8959) .. (1.4,3.9429);
 \draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions .1285 and 0.3 step 0.1245 with   {\pic[transform shape,rotate=30, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
 (n3) .. controls (4.6148,3.0594)  and(3.9718,3.285) .. (3.6391,3.5047) .. controls (3.3496,3.6104) and (3.0856,3.7212) .. (2.6522,3.8353) .. controls (2.2454,3.8856) and (1.8886,3.8959) .. (1.4,3.9429);
\draw[black, opacity=0,thin,  postaction={ decorate,  decoration={  markings,   mark=between positions 0.04 and 0.1 step 0.1245 with   {\pic[transform shape,rotate=40, scale=0.15, opacity=0.45] {car_top={blue}} ;  }}}]
 (n3) .. controls (4.6148,3.0594)  and(3.9718,3.285) .. (3.6391,3.5047) .. controls (3.3496,3.6104) and (3.0856,3.7212) .. (2.6522,3.8353) .. controls (2.2454,3.8856) and (1.8886,3.8959) .. (1.4,3.9429);
% 
\end{tikzpicture}

==> macros/packages.tex <==
%============================================================================
% The following packages can be found on http:\\www.ctan.org
% BIBTEX
\usepackage{cite}
% BIBLATEX: \usepackage[style=IEEEtran,backend=bibtex]{biblatex}

\usepackage{graphicx}  % for pdf, bitmapped graphics files
\usepackage{array}
%\usepackage{epsfig}   % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times}     % assumes new font selection scheme installed
\usepackage[fleqn]{amsmath}   % assumes amsmath package installed
\usepackage{amssymb}   % assumes amsmath package installed
%\usepackage{mathabx}   % for \widebar % Böse (font 3)
\usepackage{dsfont}
\usepackage{float}     % for placing with (H) at a specific position 
\usepackage{textgreek}
\usepackage[table]{xcolor}  % Färbige Tabellen
\usepackage{booktabs}       % Schöne Tabellen (dicke und dünne Linien)
\usepackage{filemod}        % für autoupdate bei geänderten tikz-grafiken
\usepackage{xifthen}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{footnote}
%==============================================================================
% macro for executing a shell command immidiatly 
%\newcommand{\runmycommand}[1]{\immediate\write18{#1}}
% AUTOMATIC BIBTEX
\IfFileExists{\jobname.aux}% needs --enable-write18
             {\typeout{bibtex \jobname.aux}
              \immediate\write18{bibtex \jobname.aux}
              \typeout{*** AUTO RUNNING BIBTEX ***}}
             {\typeout{*********** Rerun for bibliography *************}}
%FOR BIBLATEX %\addbibresource{./IEEEabrv,./library}
             
% Pakete für Blockdiagramme und Diagramme
\usepackage{tikz}               % Achtung die Reihenfolge der Tikz Pakete ist
\usepackage{pgfplots}           % entscheidend!
\usepackage{pgfplotstable} 
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{units}
%\usetikzlibrary{spy}
\usetikzlibrary{shadows,positioning,arrows}
%\usetikzlibrary{shapes,shapes.multipart}
\usetikzlibrary{calc}
\usetikzlibrary{trees,fit,backgrounds}
%\usetikzlibrary{patterns,decorations.pathreplacing,decorations.pathmorphing}
%\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur,shapes.symbols}

%=================================================================================
\usepgfplotslibrary{external} % PDFs machen
\tikzexternalize[prefix=tikz_temp/]     % Unterordner für PDFs
\newcommand\autoupdateexternfigure[2]{  % MAKRO UM AUTOUPDATE ZU ERMÖGLICHEN
  \tikzsetnextfilename{#2}              % pdf-filename
  \filemodCmp{#1}{tikz_temp/#2.log}%    % prüft file datum 
  {\tikzset{external/force remake=true}}% erzwingt remake wenn log alt
  {}
}
%\tikzset{external/force remake} % immer alle Bilder neu machen
% Achtung für später: EPS-Grafiken können mit Tikz auch automatisch erstellt werden (siehe Internet)
% Tipps zu eps: auf http://tex.stackexchange.com/questions/8641/export-eps-figures-from-tikz
%=================================================================================

% Spezial Worttrennungen
\hyphenation{Last-rampen Betriebs-punkt}

%============================================================================
% PDF-Einstellungen
%\usepackage[ pdfauthor={Zlatan Ajanovic, Michael Stolz, Martin Horn}
%             ,pdftitle={A Novel Observer Concept for Embedded Drivetrain Applications}
%             ,pdfpagelayout=TwoPageLeft
%             ,pdfstartview  = {FitV}
%             %,pdfpagemode  = UseAttachments %OPEN ATTACHMENTS-VIEW IN PD
%             ,pdfpagelabels = true
%             ,linkcolor     = {black}
%             ,colorlinks    = {true} 
%             ,citecolor     = {black}
%             ,urlcolor      = {black}
%             ,bookmarks, bookmarksnumbered
%             %,bookmarksopen={true}, 
%             %,pagebackref  = true, backref = page     %% turn on backreferencing
%             ,plainpages    = false
%             ,hypertexnames = true
%             ]{hyperref}
%============================================================================
% Matrizen ------------------------------------------------------------------  
%\usepackage{arydshln}         % have dotted lines to separate matrix elements 
%\newcommand{\myhdots}{\hdashline[.4pt/1.5pt]}          % macro für punktierte

==> macros/tikzStyles.tex <==
\tikzstyle{s} = [font = \footnotesize]

\tikzstyle{doppelpfeil} = [-latex,postaction={draw,shorten >=6pt,-latex}]
\tikzstyle{sarrowtip} = [>=latex]  
\tikzstyle{myarrowtip} = [>=implies] 

\tikzset{curveinscope/.style={every path/.style={draw=white, double distance=1pt, line width=2pt, double=black, text=black}}}

\DeclareRobustCommand{\myLine}[1]{
(\tikzset{external/export next=false}\begin{tikzpicture}%
\useasboundingbox (-0.2ex,0) rectangle (4.65ex,1ex);%
\draw[line width=0.3ex,#1](0,0.65ex)--(4.5ex,0.65ex);%
\end{tikzpicture})}



